Open source modelling of scenarios for a 100% renewable energy system in Barbados incorporating shore-to-ship power and electric vehicles

The high dependence on imported fuels and the potential for both climate change mitigation and economic diversification make Barbados' energy system particularly interesting for detailed transformation analysis. An open source energy system model is presented here for the analysis of a future Barbadian energy system. The model was applied in a scenario analysis, using a greenfield approach, to investigate cost-optimal and 100% renewable energy system configurations. Within the scenarios, the electrification of private passenger vehicles and cruise ships through shore-to-ship power supply was modelled to assess its impact on the energy system and the necessary investment in storage. Results show that for most scenarios of a system in 2030, a renewable energy share of over 80% is achieved in cost-optimal cases, even with a growing demand. The system's levelised costs of electricity range from 0.17 to 0.36 BBD/kWh in the cost-optimal scenarios and increase only moderately for 100% renewable systems. Under the reasonable assumption of decreasing photovoltaic investment costs, system costs of a 100% system may be lower than the current costs. The results show that pumped hydro-storage is a no-regret option for the Barbadian power system design. Overall, the results highlight the great potential of renewable energy as well as the technical and economic feasibility of a 100% renewable energy system for Barbados.

==> tables/agg_investment_cost.tex <==
\begin{table}
\centering
\caption{Aggregated investment cost in Mio. BBD per year.}
\label{tab:agg_invest_cost}
\begin{tabular}{lr}
\toprule
{} &      0 \\
\midrule
LRC      & 169.41 \\
REF      & 199.28 \\
HD-100   & 410.52 \\
MRC-100  & 251.05 \\
RB-100   & 355.99 \\
EVUC     & 197.97 \\
RB       & 197.27 \\
HD       & 246.89 \\
REF-100  & 293.11 \\
HBC-100  & 393.78 \\
MRC      & 196.69 \\
NPHS-100 & 307.66 \\
NPHS     & 196.68 \\
SQ-100   & 192.60 \\
EVUC-100 & 307.29 \\
SQ       & 126.19 \\
LRC-100  & 212.65 \\
LOP-100  & 293.11 \\
HBC      & 204.76 \\
LOP      & 129.34 \\
\bottomrule
\end{tabular}
\end{table}


==> tables/carrier_cost.tex <==
\begin{table}
\centering
\caption{Cost of energy carriers in different scenarios}
\label{tab:carrier_cost}
\begin{tabular}{llrr}
\toprule
        &      &  Cost (BBD/MWh) &  CO\textbackslash textsubscript\{2\} (t/MWh) \\
name & carrier\_scenario &                 &                              \\
\midrule
diesel & base &          153.55 &                         0.27 \\
hfo & base &          118.33 &                         0.29 \\
waste & base &           22.93 &                         0.00 \\
bagasse & base &           22.93 &                         0.00 \\
\bottomrule
\end{tabular}
\end{table}


==> tables/energy.tex <==
\begin{table}
\centering
\caption{Energy supply and demand in GWh.}
\label{tab:energy}
\begin{tabular}{lp{1.3cm}p{1.3cm}p{1.3cm}p{1.3cm}p{1.3cm}p{1.3cm}p{1.3cm}p{1.3cm}p{1.3cm}p{1.3cm}p{1.3cm}p{1.3cm}p{1.3cm}p{1.3cm}p{1.3cm}}
\toprule
{} &  hfo-lsce &  hfo-msce &  solar-pv-distributed &  solar-pv-utility &  wind-onshore &  bagasse-st &  waste-ocgt &   demand &  ev-demand &  excess &  phs-cos &    phs &  battery-cos &  battery \\
\midrule
SQ       &    134.54 &     14.63 &                  0.00 &             32.84 &        671.44 &      166.04 &        0.00 &  -943.00 &       0.00 &  -70.64 &   -29.31 &  23.45 &         0.00 &     0.00 \\
SQ-100   &      0.00 &      0.00 &                  0.00 &            136.07 &        664.91 &      166.04 &       74.26 &  -943.00 &       0.00 &  -89.76 &   -42.63 &  34.11 &         0.00 &     0.00 \\
HD       &    272.72 &     38.81 &                  0.00 &            138.52 &       1171.65 &      166.04 &        0.00 & -1321.27 &    -265.43 & -140.37 &   -82.66 &  66.13 &         0.00 &     0.00 \\
HD-100   &      0.00 &      0.00 &                347.67 &            138.52 &       1177.13 &      166.04 &       74.26 & -1321.27 &    -265.43 & -163.08 &  -196.17 &  86.47 &        -0.00 &     0.00 \\
RB       &    227.36 &     33.57 &                  0.00 &            138.52 &        900.26 &       83.02 &        0.00 &  -943.00 &    -265.43 & -116.38 &   -68.92 &  55.14 &         0.00 &     0.00 \\
RB-100   &      0.00 &      0.00 &                395.45 &            138.52 &        857.56 &       83.02 &       37.13 &  -943.00 &    -265.43 & -125.26 &  -219.52 &  85.66 &         0.00 &     0.00 \\
REF      &    167.72 &     34.08 &                  0.00 &            138.52 &        853.04 &      166.04 &        0.00 &  -943.00 &    -265.43 &  -91.90 &   -74.17 &  59.34 &        -1.04 &     0.93 \\
REF-100  &      0.00 &      0.00 &                 46.43 &            138.52 &       1033.63 &      166.04 &       74.26 &  -943.00 &    -265.43 & -125.26 &  -178.58 &  98.36 &        -8.36 &     7.52 \\
NPHS     &    181.10 &     37.22 &                  0.00 &            138.52 &        841.41 &      166.04 &        0.00 &  -943.00 &    -265.43 & -107.02 &     0.00 &   0.00 &       -47.05 &    42.35 \\
NPHS-100 &      0.00 &      0.00 &                218.23 &            138.52 &        818.57 &      166.04 &       74.26 &  -943.00 &    -265.43 & -125.26 &     0.00 &   0.00 &       -79.48 &    41.69 \\
EVUC     &    185.60 &     47.81 &                  0.00 &              0.00 &        989.90 &      166.04 &        0.00 &  -943.00 &    -265.43 & -113.08 &  -109.65 &  87.72 &       -17.85 &    16.06 \\
EVUC-100 &      0.00 &      0.00 &                  0.00 &            138.52 &       1116.22 &      166.04 &       74.26 &  -943.00 &    -265.43 & -125.26 &  -246.80 & 132.51 &       -29.29 &    26.36 \\
LOP      &    586.66 &     92.48 &                  0.00 &             28.13 &        571.65 &        0.00 &        0.00 &  -943.00 &    -265.43 &  -26.34 &     0.00 &   0.00 &         0.00 &     0.00 \\
LOP-100  &      0.00 &      0.00 &                 46.43 &            138.52 &       1033.63 &      166.04 &       74.26 &  -943.00 &    -265.43 & -125.26 &  -182.55 & 102.33 &        -8.36 &     7.52 \\
LRC      &     61.78 &     20.10 &                405.36 &            138.52 &        532.97 &      166.04 &        0.00 &  -943.00 &    -265.43 &  -56.10 &   -69.75 &  55.80 &       -21.48 &    19.33 \\
LRC-100  &      0.00 &      0.00 &                405.36 &            138.52 &        686.44 &      166.04 &        0.00 &  -943.00 &    -265.43 & -124.92 &   -94.36 &  75.49 &         0.00 &     0.00 \\
MRC      &     90.70 &     21.13 &                311.76 &            138.52 &        595.75 &      166.04 &        0.00 &  -943.00 &    -265.43 &  -60.97 &   -43.89 &  35.11 &       -15.84 &    14.26 \\
MRC-100  &      0.00 &      0.00 &                405.36 &            138.52 &        686.44 &      166.04 &        0.00 &  -943.00 &    -265.43 & -124.92 &   -94.36 &  75.49 &        -0.00 &     0.00 \\
HBC      &    364.72 &     32.66 &                  0.00 &            138.52 &        790.62 &        0.00 &        0.00 &  -943.00 &    -265.43 &  -63.81 &   -50.72 &  40.58 &         0.00 &     0.00 \\
HBC-100  &      0.00 &      0.00 &                208.73 &            138.52 &        766.55 &      166.04 &       74.26 &  -943.00 &    -265.43 &  -85.98 &   -77.77 &  62.22 &         0.00 &     0.00 \\
\bottomrule
\end{tabular}
\end{table}


==> tables/installed_capacities.tex <==
\begin{table}
\centering
\caption{Installed capacities in MW.}
\label{tab:installed_capacities}
\begin{tabular}{lrrrrrrrrr}
\toprule
Tech &  bagasse-st &  hfo-lsce &  hfo-msce &  hydro-phs &  lithium-battery &  pv-distributed &  pv-utility &  waste-ocgt &  wind-onshore \\
Scenario &             &           &           &            &                  &                 &             &             &               \\
\midrule
EVUC     &       30.59 &     78.51 &     97.02 &      64.74 &            16.90 &            0.00 &        0.00 &        0.00 &        312.27 \\
EVUC-100 &       87.67 &      0.00 &      0.00 &     152.17 &            29.76 &            0.00 &       80.00 &       16.22 &        352.11 \\
HBC      &        0.00 &    105.53 &     98.35 &      43.01 &             0.00 &            0.00 &       80.00 &        0.00 &        249.40 \\
HBC-100  &       72.14 &      0.00 &      0.00 &     121.00 &             0.00 &          120.54 &       80.00 &       16.68 &        241.81 \\
HD       &       30.25 &    100.78 &    113.12 &      54.62 &             0.00 &            0.00 &       80.00 &        0.00 &        369.60 \\
HD-100   &       96.13 &      0.00 &      0.00 &     134.80 &             0.00 &          200.78 &       80.00 &       17.98 &        371.33 \\
LOP      &        0.00 &    122.92 &    148.35 &       0.00 &             0.00 &            0.00 &       16.24 &        0.00 &        180.33 \\
LOP-100  &       84.62 &      0.00 &      0.00 &     124.38 &            11.61 &           26.81 &       80.00 &       15.75 &        326.06 \\
LRC      &       34.41 &     30.85 &     60.05 &      36.75 &            15.65 &          234.10 &       80.00 &        0.00 &        168.13 \\
LRC-100  &       81.10 &      0.00 &      0.00 &      95.06 &             0.00 &          234.10 &       80.00 &        0.00 &        216.54 \\
MRC      &       32.63 &     40.36 &     82.76 &      26.23 &            11.51 &          180.04 &       80.00 &        0.00 &        187.93 \\
MRC-100  &       81.10 &      0.00 &      0.00 &      95.06 &             0.00 &          234.10 &       80.00 &        0.00 &        216.54 \\
NPHS     &       31.26 &     69.35 &     90.60 &       0.00 &            55.59 &            0.00 &       80.00 &        0.00 &        265.42 \\
NPHS-100 &       90.51 &      0.00 &      0.00 &       0.00 &           101.03 &          126.03 &       80.00 &       16.08 &        258.22 \\
RB       &       15.01 &     81.95 &    101.69 &      48.04 &             0.00 &            0.00 &       80.00 &        0.00 &        283.99 \\
RB-100   &       60.45 &      0.00 &      0.00 &     143.69 &             0.00 &          228.38 &       80.00 &       11.10 &        270.52 \\
REF      &       30.59 &     66.75 &    102.34 &      46.03 &             1.07 &            0.00 &       80.00 &        0.00 &        269.10 \\
REF-100  &       84.62 &      0.00 &      0.00 &     124.38 &            11.61 &           26.81 &       80.00 &       15.75 &        326.06 \\
SQ       &       30.89 &     51.76 &     24.59 &      18.36 &             0.00 &            0.00 &       18.97 &        0.00 &        211.81 \\
SQ-100   &       74.84 &      0.00 &      0.00 &      36.78 &             0.00 &            0.00 &       78.58 &       13.98 &        209.75 \\
\bottomrule
\end{tabular}
\end{table}


==> tables/investment_cost.tex <==
\begin{table}
\centering
\caption{Annualised investment cost per technology for all scenarios in Mio. BBD.}
\label{tab:investment_cost}
\begin{tabular}{lp{1.2cm}p{1.2cm}p{1.2cm}p{1.2cm}p{1.2cm}p{1.2cm}p{1.2cm}p{1.2cm}p{1.2cm}}
\toprule
{} &  hfo-lsce &  hfo-msce &  solar-pv-distributed &  solar-pv-utility &  wind-onshore &  lithium-battery &  hydro-phs &  bagasse-st &  waste-ocgt \\
\midrule
LRC      &      7.38 &     12.93 &                 46.87 &             11.44 &         47.86 &             4.93 &      13.64 &       24.36 &        0.00 \\
REF      &     15.96 &     22.03 &                  0.00 &             29.75 &         92.46 &             0.34 &      17.08 &       21.66 &        0.00 \\
HD-100   &      0.00 &      0.00 &                103.37 &             29.75 &        127.58 &             0.00 &      50.03 &       68.06 &       31.73 \\
MRC-100  &      0.00 &      0.00 &                 70.30 &             17.16 &         70.89 &             0.00 &      35.28 &       57.41 &        0.00 \\
RB-100   &      0.00 &      0.00 &                117.57 &             29.75 &         92.95 &             0.00 &      53.34 &       42.79 &       19.60 \\
EVUC     &     18.78 &     20.89 &                  0.00 &              0.00 &        107.29 &             5.32 &      24.03 &       21.66 &        0.00 \\
RB       &     19.60 &     21.89 &                  0.00 &             29.75 &         97.58 &             0.00 &      17.83 &       10.63 &        0.00 \\
HD       &     24.10 &     24.35 &                  0.00 &             29.75 &        126.99 &             0.00 &      20.27 &       21.42 &        0.00 \\
REF-100  &      0.00 &      0.00 &                 13.80 &             29.75 &        112.03 &             3.66 &      46.17 &       59.91 &       27.80 \\
HBC-100  &      0.00 &      0.00 &                 65.12 &             26.53 &        112.33 &             0.00 &      44.91 &      115.44 &       29.45 \\
MRC      &      9.65 &     17.82 &                 54.07 &             17.16 &         61.53 &             3.63 &       9.74 &       23.10 &        0.00 \\
NPHS-100 &      0.00 &      0.00 &                 64.88 &             29.75 &         88.72 &            31.84 &       0.00 &       64.08 &       28.39 \\
NPHS     &     16.59 &     19.51 &                  0.00 &             29.75 &         91.20 &            17.52 &       0.00 &       22.13 &        0.00 \\
SQ-100   &      0.00 &      0.00 &                  0.00 &             29.22 &         72.07 &             0.00 &      13.65 &       52.98 &       24.68 \\
EVUC-100 &      0.00 &      0.00 &                  0.00 &             29.75 &        120.98 &             9.38 &      56.48 &       62.07 &       28.63 \\
SQ       &     12.38 &      5.29 &                  0.00 &              7.05 &         72.77 &             0.00 &       6.81 &       21.87 &        0.00 \\
LRC-100  &      0.00 &      0.00 &                 46.87 &             11.44 &         61.65 &             0.00 &      35.28 &       57.41 &        0.00 \\
LOP-100  &      0.00 &      0.00 &                 13.80 &             29.75 &        112.03 &             3.66 &      46.17 &       59.91 &       27.80 \\
HBC      &     25.24 &     21.18 &                  0.00 &             26.53 &        115.86 &             0.00 &      15.96 &        0.00 &        0.00 \\
LOP      &     29.40 &     31.94 &                  0.00 &              6.04 &         61.96 &             0.00 &       0.00 &        0.00 &        0.00 \\
\bottomrule
\end{tabular}
\end{table}


==> tables/lcoe.tex <==
\begin{table}
\centering
\caption{LCOE in BBD per kWh for all scenarios.}
\label{tab:lcoe}
\begin{tabular}{lrr}
\toprule
{} &  COPT &  100RE \\
\midrule
SQ   &  0.20 &   0.23 \\
HD   &  0.21 &   0.27 \\
RB   &  0.22 &   0.29 \\
REF  &  0.22 &   0.25 \\
NPHS &  0.22 &   0.26 \\
EVUC &  0.22 &   0.26 \\
LOP  &  0.18 &   0.25 \\
LRC  &  0.17 &   0.18 \\
MRC  &  0.20 &   0.21 \\
HBC  &  0.25 &   0.33 \\
\bottomrule
\end{tabular}
\end{table}


==> tables/re_share.tex <==
\begin{table}
\centering
\caption{Renewable energy share in different scenarios.}
\label{tab:re_share}
\begin{tabular}{lr}
\toprule
{} &    0 \\
\midrule
EVUC     & 0.81 \\
EVUC-100 & 1.00 \\
HBC      & 0.68 \\
HBC-100  & 1.00 \\
HD       & 0.81 \\
HD-100   & 1.00 \\
LOP      & 0.46 \\
LOP-100  & 1.00 \\
LRC      & 0.93 \\
LRC-100  & 1.00 \\
MRC      & 0.91 \\
MRC-100  & 1.00 \\
NPHS     & 0.83 \\
NPHS-100 & 1.00 \\
RB       & 0.79 \\
RB-100   & 1.00 \\
REF      & 0.84 \\
REF-100  & 1.00 \\
SQ       & 0.84 \\
SQ-100   & 1.00 \\
\bottomrule
\end{tabular}
\end{table}


==> tables/tech_data.tex <==
\begin{table}
\centering
\caption{Cost and technical data for supply units. All costs are in BB\$.}
\label{tab:tech_data}
\begin{tabular}{llp{1.5cm}p{1.5cm}p{1cm}p{1cm}p{0.75cm}p{1.5cm}}
\toprule
      &      &  capex (\$/kW) &  lifetime (a) &  wacc (-) &  eta (\%) &  fom (\%) &  vom (\$/MWh) \\
carrier & tech &               &               &           &          &          &              \\
\midrule
wind & onshore &        3500.0 &            20 &      0.07 &    100.0 &      4.0 &            0 \\
solar & pv-distributed &        5400.0 &            20 &      0.07 &    100.0 &      1.0 &            0 \\
      & pv-utility &        3900.0 &            20 &      0.07 &    100.0 &      1.0 &            0 \\
lithium & battery &         100.0 &            12 &      0.07 &     94.9 &      3.0 &            0 \\
hydro & phs &        5000.0 &            45 &      0.07 &     89.4 &      1.0 &            0 \\
hfo & lsce &        2853.0 &            30 &      0.07 &     46.4 &      4.0 &           12 \\
      & msce &        2344.0 &            25 &      0.07 &     43.9 &      7.0 &           18 \\
bagasse & st &        8000.0 &            25 &      0.07 &     25.3 &      3.1 &           15 \\
waste & ocgt &       18000.0 &            20 &      0.07 &     34.1 &      3.9 &           15 \\
\bottomrule
\end{tabular}
\end{table}


==> tables/total_dispatchable_capacity.tex <==
\begin{table}
\centering
\caption{Peak demand and total dispatchable capacity in MW for all scenarios.}
\label{tab:energy}
\begin{tabular}{lrrr}
\toprule
{} &  Peak Demand in MW &  Dispatchable Capacity in MW &  Share in \% \\
\midrule
SQ       &             132.43 &                       125.60 &        0.95 \\
SQ-100   &             132.43 &                       125.60 &        0.95 \\
HD       &             355.04 &                       298.77 &        0.84 \\
HD-100   &             355.04 &                       248.91 &        0.70 \\
RB       &             302.45 &                       246.69 &        0.82 \\
RB-100   &             302.45 &                       215.25 &        0.71 \\
REF      &             302.45 &                       246.78 &        0.82 \\
REF-100  &             302.45 &                       236.36 &        0.78 \\
NPHS     &             302.45 &                       246.80 &        0.82 \\
NPHS-100 &             302.45 &                       207.63 &        0.69 \\
EVUC     &             317.20 &                       287.76 &        0.91 \\
EVUC-100 &             317.20 &                       285.83 &        0.90 \\
LOP      &             302.45 &                       271.27 &        0.90 \\
LOP-100  &             302.45 &                       236.36 &        0.78 \\
LRC      &             302.45 &                       177.71 &        0.59 \\
LRC-100  &             302.45 &                       176.16 &        0.58 \\
MRC      &             302.45 &                       193.48 &        0.64 \\
MRC-100  &             302.45 &                       176.16 &        0.58 \\
HBC      &             302.45 &                       246.89 &        0.82 \\
HBC-100  &             302.45 &                       209.82 &        0.69 \\
\bottomrule
\end{tabular}
\end{table}

